Perturb Your Data: Paraphrase-Guided Training Data Watermarking

Training data detection is critical for enforcing copyright and data licensing, as Large Language Models (LLM) are trained on massive text corpora scraped from the internet. We present SPECTRA, a watermarking approach that makes training data reliably detectable even when it comprises less than 0.001% of the training corpus. SPECTRA works by paraphrasing text using an LLM and assigning a score based on how likely each paraphrase is, according to a separate scoring model. A paraphrase is chosen so that its score closely matches that of the original text, to avoid introducing any distribution shifts. To test whether a suspect model has been trained on the watermarked data, we compare its token probabilities against those of the scoring model. We demonstrate that SPECTRA achieves a consistent p-value gap of over nine orders of magnitude when detecting data used for training versus data not used for training, which is greater than all baselines tested. SPECTRA equips data owners with a scalable, deploy-before-release watermark that survives even large-scale LLM training.

==> tables/analysis.tex <==
\begin{table}[h!]
\centering
\caption{Percentage of documents for which \minkpp scores increase after training. WM refers to watermarked.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccccccc}
\hline
 \multicolumn{2}{c}{\textbf{PubMed}} 
& \multicolumn{2}{c}{\textbf{Wiki}} 
& \multicolumn{2}{c}{\textbf{HN}} 
& \multicolumn{2}{c}{\textbf{PeS2o}} \\
\cline{1-8}
\textbf{WM} & \textbf{Orig} 
& \textbf{WM} & \textbf{Orig} 
& \textbf{WM} & \textbf{Orig} 
& \textbf{WM} & \textbf{Orig} \\
\hline
 36.0\% & 16.6\% & 28.4\% & 19.2\% & 48.8\% & 7.4\% & 50.9\% & 44.4\% \\
\hline
\end{tabular}}

\label{tab:analysis}
\end{table}



==> tables/ration_per.tex <==
\begin{table}[htbp]
\centering
\caption{\% of points for which $Ratio_N$ is higher than $Ratio_D$}
\label{tab:ratio}
\begin{tabular}{@{}llcccc@{}}
\toprule
& \textbf{PubMed} & \textbf{Wiki} & \textbf{HN} & \textbf{PeS2o}\\
\midrule
Perc & 68.3\% & 70.4\% & 68.4\% & 50.9\% \\
\bottomrule
\end{tabular}
\end{table}
